NIR-probe transient absorption on rubrene microcavities demonstrates no changes to singlet fission by strong coupling

Strong light-matter coupling has been proposed to control singlet-exciton fission, yet reported effects remain controversial due to the prevalence of cavity-induced optical artifacts in transient absorption measurements. Here, we investigate singlet fission in dielectric microcavities containing rubrene by probing in the near-infrared region, outside the cavity stopband, to eliminate mode-filtering artifacts. Across contrasting cavity quality factors ($Q = 90$ and $1150$) and a range of exciton-photon detunings ($+20$ to $-110$ meV), we find that the underlying kinetics are virtually identical to uncoupled films. Although minor spectral changes occur, transfer matrix simulations reveal these stem purely from mirror interference rather than modified photophysics. Transient electron paramagnetic resonance further confirms that high-spin triplet dynamics remain unperturbed. Together, these findings establish a widely applicable experimental framework for evaluating molecular photophysics in microcavities, revealing that singlet fission remains unaltered in strongly coupled rubrene.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "pdflatex -interaction=batchmode -shell-escape \"$_[0]\"" );
    }
}
